A Successive-Elimination Approach to Adaptive Robotic Sensing

We study an adaptive source seeking problem, in which a mobile robot must identify the strongest emitter(s) of a signal in an environment with background emissions. Background signals may be highly heterogeneous and can mislead algorithms that are based on receding horizon control. We propose AdaSearch, a general algorithm for adaptive source seeking in the face of heterogeneous background noise. AdaSearch combines global trajectory planning with principled confidence intervals in order to concentrate measurements in promising regions while guaranteeing sufficient coverage of the entire area. Theoretical analysis shows that AdaSearch confers gains over a uniform sampling strategy when the distribution of background signals is highly variable. Simulation experiments demonstrate that when applied to the problem of radioactive source seeking, AdaSearch outperforms both uniform sampling and a receding time horizon information-maximization approach based on the current literature. We also demonstrate AdaSearch in hardware, providing further evidence of its potential for real-time implementation.

==> algorithm_info_max.tex <==
%!TEX root = main.tex

\begin{algorithm}[t]
  \textbf{Input} initial information vector $\mbf{y}(t_0)$ and information matrix
  $\mbf{Y}(t_0)$, planning horizon $T_{\text{plan}}$, sensitivity function
  $h(\cdot, \cdot)$, box $\mc{B}$, sensor position $p(\cdot)$ \\
  \textbf{While} True \\
  \Indp \textbf{If} stopping condition satisfied, \textbf{Break} \\
  \textbf{If} new sensor measurement \\
  \Indp \textbf{Update} $\mbf{y}(t)$ and $\mbf{Y}(t)$ as in
  \eqref{eqn:info_vec_update}, \eqref{eqn:info_mat_update} \\
  \Indm \textbf{If} nearing the end of planned trajectory \\
  \Indp \textbf{Replan} trajectory $\tau$ to maximize information objective in
  \eqref{eqn:info_max} \\
  \Indm \Indm \textbf{Return} $\arg \max_x \bm{\hat \mu}_x(t)$ and $\max_x
  \bm{\hat \mu}_x(t)$
  \caption{$\infomax$ (Baseline)  \label{alg:info_max}}
\end{algorithm}


==> analysis.tex <==
% !TEX root = main_nips.tex





%Algorithm \ref{snake_lucb++} presents $\snakeucb$, a general framework for
%locating the set $\Sstk$ in a discrete environment $\calS$. For each round $i$, we
%maintain a set of points $\Stop_i$ which we are confident are among the top-$k$,
%and a set of candidate points $\calSi$ about which we are still uncertain. The
%remaining points $\calS \setminus \{\Stop_i \cup \calSi\}$ are confidently not
%among the top-$k$.
%This confidence is expressed in terms of lower and upper confidence intervals,
%$\LCB_i(x)$ and $\UCB_i(x)$ for all points $x \in \calSi$ and rounds $i$, which are constructed to
%satisfy the coverage guarantee $\LCB_i(x) \le \mu(x) \le \UCB_i(x)$ with high
%probability.

%remaining points $\calS \setminus \{\Stop_i \cup \calSi\}$ are confidently not
%among the top-$k$.
%This confidence is expressed in terms of lower and upper confidence intervals,
%$\LCB_i(x)$ and $\UCB_i(x)$ for all points $x \in \calSi$ and rounds $i$, which are constructed to
%satisfy the coverage guarantee $\LCB_i(x) \le \mu(x) \le \UCB_i(x)$ with high
%probability.


%The goal of $\snakeucb$ sequence of configurations $(z(t)) \subset \config$
%, along with timing patterns,
%which together specify a sensing trajectory which
%from the agent can quickly identify $S^*(k)$. At its core, the algorithm procee

%$\snakeucb$ takes as input an ordering over configuraitons, $\trajpoints = z^{(1)},z^{(2)},...,z^{(n)}$, where every configuration in $\config$ is visited. The ordering is chosen to reduce total travel time between configurations in each round. For omnidirectional sensors and topologically simple configuration sets $\config$, a
%simple ``snake'' pattern (Fig.~\ref{fig:snake_pattern}) suffices; more intricate
%cases are discussed below.





%\input{theorem_and_baby_proof}

% \esther{extensions are outdated now.} \textbf{Extensions.} $\snakeucb$ readily
% extends to the problem of finding the $k$ strongest sources. This may be
% accomplished by
% % replacing the termination criteria in
% % Line~\ref{alg:termination_criterion} with $|S_i| = k$, and replacing $\{x
% % \in
% % \calS_i | \UCB_{i+1}(x) \geq \LCB_{i+1}\}$ in the pruning step on
% % Line~\ref{alg:prune_step} with the set of all points $x \in \calS_i$ for
% % which
% % the $\UCB$ of $x$ is greater than or equal to the $k^{th}$ largest $\LCB$ of
% % candidate points in $\calS_i$. For full optimality, we would ignore points
% % that are already definitely in the top-k set (i.e. don't resample points for
% % which $\LCB(x)$ is greater than the $k+1^{th}$ highest $\UCB$).
% maintaining one set of candidate points and another set of points that are
% confidently amongst the top-$k$ sources. The algorithm terminates when the set
% of candidate top-$k$ sources has cardinality $k$. Further details of the
% top-$k$ algorithm and its sample complexity are provided in the appendix.

% % For $k$ source identification, the sample
% % complexity changes from depending on the sum of the gaps $\mu(x^*)/(\mu(x) -
% % \mu(x^*))^2$ to the sum of the gaps $\mu(x_k)/(\mu(x_-) - \mu(x_k))^2$ for
% % all
% % $x_-$ with $\mu(x_-) < \mu(x_k)$, and $\mu(x_{+})/(\mu(x_+) -
% % \mu(x_{k+1}))^2$
% % for all $x_+$ with $\mu(x_+) > \mu(x_{k+1})$; here $\mu(x_{k})$ and
% % $\mu(x_{k+1})$ denote the means of the $k$-th and $k$-largest pixels,
% % respectively.

% Extensions to precision mapping and to discerning whether each source
% intensity is above or below a given threshold $\{ \mu(x) >
% \mu_{\textrm{thresh}} : \forall x \in \calS\}$ are also straightfoward, and
% highlight a pitfall of the pointwise sensing model. In threshold detection,
% for example, the stopping condition would be to terminate when all $|\calS|$
% confidence intervals are small enough to exclude the value
% $\mu_{\textrm{thresh}} $. Under the pointwise sensing model measurements can
% be uniquely attributed to the nearest source; hence an optimal algorithm could
% hover at each point $x$ until the confidence interval $(\LCB(x), \UCB(x))$
% does not contain $\mu_{\textrm{thresh}}$ before moving on to the next point
% $x'' \in \calS$. However, under the physical sensing model this approach would
% lead to the rows of the sensitivity matrix $H$ being nearly collinear (and
% hence making $H$ ill-conditioned and at least some confidence intervals large)
% until relatively late in the trajectory. Thus, even in the mapping scenario,
% the travel time between points in the iterative ``snake'' pattern serves the
% practical purpose of improving the conditioning of $H$ and hence
% disambiguating the counts attributable to different sources.


==> conf_interval.tex <==
%!TEX root = analysis_main.tex
\section{Poisson Confidence Intervals\label{sec:conf_interval}}



==> methods.tex <==
%!TEX root = main_nips.tex



\section{Case Study: Radioactive Source Seeking ($\RSS$)}
\label{sec:methods}
Here we detail an instantiation of $\snakeucb$ for the radioactive source-seeking ($\RSS$) problem with an omnidirectional, perfectly absorbing
sensor onboard a quadrotor helicopter.
%
We use the Poisson sensing model~\eqref{eq:Poisson_sensing} described in Sec.~\ref{sec:algorithm_snake}.
%
For
radioactive sources, $\mu(x)$ corresponds to intensity of emissions, and physical laws allow us to approximate the sensitivity function by $h(x,z) :=
c/ \|x - z\|_2^2$ for some constant $c$.
%
To demonstrate the effectiveness of $\snakeucb$, we compare to two baselines: a uniform-sampling based algorithm $\naivesnake$ (also in Sec.~\ref{sec:algorithm_snake}) and a spatially-greedy information maximization algorithm $\infomax$.




\textbf{Confidence Intervals for $\RSS$.} With this forward model, the MLE
for the estimated Poisson counts is in general nontrivial, but we can
approximate it in the limit: $ \frac{1}{\sqrt{\tau}}\Poi(\tau\mu)
\overset{d}{\rightarrow} \normal{\mu, \mu} $ as $\tau \rightarrow \infty$. Using
this simplification, we may compute $\hat{\mu}$ as the least squares solution:
\begin{equation}
  \label{eqn:lstsq}
  \hat{\mu} = \arg\min_{\mu} \| H \mu - y \|_2^2~,
\end{equation}
where $y \in \RR^m$ is a vector representing the number of counts at each of $m$
time intervals of duration $\tau$, and $H \in \RR^{m \times |\calS| }$ is a
rescaled sensitivity matrix such that $H_{jk}$ gives the measurement-adjusted sensitivity $h$ of the sensor to the
point $x_k \in \calS$ at measurement $j$ taken from orientation $z(j)$, i.e.
$H_{jk} = h(x_k, z(j)) / (y_j + b)$. The rescaling term $y_j + b$ is a plug-in
estimator for the variance of measurement $y_j$ (with small bias $b$ introduced
for numerical stability). In order to attribute components of
the signal $y$ to individual emitters $x$, this model of the sensing process
requires measurements to be taken from different locations; otherwise, $H$ will
be rank-deficient or ill-conditioned. The confidence bounds are given by the
standard Gaussian confidence bounds
\begin{equation}
  \label{eqn:cis}
  \LCB(x_k), \UCB(x_k) := \hat{\mu}(x_k) \pm \alpha(\delta) \cdot\Sigma^{1/2}_{kk}, \textnormal{where\ } \Sigma := (H^\top H)^{-1} \enspace ,
\end{equation}
where $\alpha(\delta)$ controls the confidence width as a function of desired probability of error $\delta$. We remark that $\Sigma$ implicitly captures the effect of the plug-in mean estimate $y_i$ on the variance estimate. We use a Kalman
filter to solve the least squares problem in \eqref{eqn:lstsq}
and obtain the confidence intervals in \eqref{eqn:cis}.

% Concretely, we approximate each new sensor measurement (photon count) $y \in
% \mbb{N}$ as approximately Gaussian, i.e. $y \sim \normal{\expect{y},
% \expect{y} + b}$.\footnote{We use a plug-in estimator for $\expect{y}$, i.e.
% $\expect{y} \approx y$, and set the small bias term $b = 10$ to improve
% numerical stability.}

\textbf{Design and planning for $\snakeucb$.} Because this sensitivity function $h$
follows an inverse-square law, the most informative measurements about $\mu(x)$
are those taken at configurations $z$ near to $x$. Hence, we use the same design and planning
strategy as in the point-wise measurement model, with a one meter vertical offset between configurations $z$ and points $x$ on the ground. Specifically, we follow the
snake pattern (Fig.~\ref{fig:snake_pattern}), slowing down over all $x \in \calS_i$.

\begin{figure}[htbp] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=.4\linewidth]{figures/snake_small.pdf} 
    \caption{``Snake'' trajectory shown with a grid of size $6 \times 6$. The
      trajectory ensures that each point in the grid is covered at some point
      during each circuit.}
    \label{fig:snake_pattern}
\end{figure}


% \subsection{Approximate Confidence Intervals}
% \label{subsec:approx_confidence_intervals}

% We maintain estimated gamma emission rates using the Kalman filter
% \cite{kalman1960new}, which tracks both the means and covariances of the
% estimated emissions at each pixel. The Kalman filter is the optimal mean
% square estimator when the true emission rates $\{ \mu_x \}$ evolve linearly
% over time and measurements are linear, in the presence of independent Gaussian
% process and measurement noise. These linearity assumptions hold in our case,
% as emission rates are static, and as per \eqref{eqn:sensor_rate}, expected
% measurements are linear in $\{ \mu_x \}$. Although sensor measurements are
% Poisson-distributed as described in Sec. \ref{subsec:emission_sensing_models},
% measurements from high-emitting sources will appear to be approximately
% Gaussian. This approximation will hold as long as the quadrotor does not stray
% too far from the grid. We choose to make these approximations because our
% application demands a computationally efficient method that is able to reason
% about confidence intervals in real time. We expect that the performance of
% $\snakeucb$ would only improve if the underlying radiation intensity estimator
% were more precise. Moreover, these approximations are accurate enough that in
% all of our experiments (Sec. \ref{sec:results}), all three algorithms
% correctly locate the source.

% Because emission rates $\bm{\mu} \triangleq [\mu_1, \dots, \mu_N]^\top$ are
% static, it is computationally efficient to use the information form of the
% Kalman filter. Indexing by time $t$ then, for measurement $z(t)$, measurement
% variance $\sigma^2(t)$, sensitivity vector $\mbf{h}(t)$, information vector
% $\mbf{y}(t)$, and information matrix $\mbf{Y}(t)$, the update is
% \begin{align}
%   \label{eqn:info_vec_update}
%   \mbf{y}(t) &= \mbf{y}(t - T_{\text{exposure}}) + \mbf{h}(t)^\top z(t) /
%     %   \sigma^2(t) \\
%  \label{eqn:info_mat_update}
%  \mbf{Y}(t) &= \mbf{Y}(t - T_{\text{exposure}}) + \mbf{h}(t)^\top \mbf{h}(t) /
%    %  \sigma^2(t)
% \end{align}

% Since the measurement $z(t)$ is actually Poisson-distributed with variance
% depending upon both $\mbf{h}(t)$ and the unknown $\bm{\mu}$, we approximate
% the variance of $z(t)$ by $z(t)$ itself. However, even though $\sigma^2(t) =
% z(t)$ is an unbiased estimator, we introduce a small bias term $b$ (i.e.
% $\sigma^2(t) = z(t) + b$) to avoid divide-by-zero issues and to aid the filter
% in recovering from small, noisy measurements.\footnote{For all experiments in
% this paper, $b=10$. }

% We convert the information vector and matrix back to the Kalman mean estimator
% $\bm{\hat \lambda}(t)$ and covariance matrix $\bm{\hat \Sigma}(t)$ as follows:
% \begin{align}
%   \label{eqn:info_vec_conversion}
%   \bm{\hat \lambda}(t) &= \mbf{Y}(t)^{-1} \mbf{y}(t) \\
%   \label{eqn:info_mat_conversion}
%   \bm{\hat \Sigma}(t) &= \mbf{Y}(t)^{-1}
% \end{align}
% We can then use these mean and covariance estimates to generate upper
% ($\text{UCB}_x(t)$) and lower ($\text{LCB}_x(t)$) confidence bounds for pixel
% $x$ at time $t$:
% \begin{align}
%   \label{eqn:ucb}
%   \text{UCB}_x(t) &= \bm{\hat \lambda}(t)_x + \xi \sqrt{\bm{\hat \Sigma}(t)_{xx}} \\
%   \label{eqn:lcb}
%   \text{LCB}_x(t) &= \bm{\hat \lambda}(t)_x - \xi \sqrt{\bm{\hat \Sigma}(t)_{xx}}
% \end{align}
% where the parameter $\xi$ controls the width of the confidence interval and
% may be computed to match a desired false positive rate $\alpha$.

% In contrast, this assumption is less applicable for the background radiation
% emitting pixels; however, since we ultimately compare a single large value
% cell with several smaller ones, this is unlikely to be an issue
% [\EstherNote{not sure if I believe this!}] Unlike Poisson estimates, Gaussian
% estimates will allow for confidence intervals which may contain negative
% values; in this case we clip the interval at zero.

% \subsection{Baseline Algorithms}
% \label{subsec:baseline_algorithms}

% \subsubsection{$\infomax$}
% \label{subsubsec:info_max}

% \input{algorithm_info_max}

\textbf{$\naivesnake$ algorithm.} As a non-adaptive baseline, we implement a
uniform sampling scheme that follows the ``snake'' trajectory in
Fig.~\ref{fig:snake_pattern} at constant speed. This global $\naivesnake$ trajectory
results in sensitive measurements uniformly spread over the grid, and avoids
redundant movements.

\textbf{$\infomax$ algorithm.} As discussed in Sec. \ref{sec:related_work}, one
of the most successful methods for active search in robotics is receding horizon informative
path planning, e.g. \cite{marchant2014bayesian, martinez2009bayesian}.
% Ideally, such planning schemes lead to trajectories that spend most of their
% time in regions where measurements reveal information about the parameters to
% be estimated. Because measurements collected in higher-emission regions have
% greater variance under the Poisson model, we expect $\infomax$ to spend the
% more of its time in these promising regions. However, the myopic planning
% horizon can cause the planner to be inefficient over long time scales.
% Comparing this class of methods to $\naivesnake$ and $\snakeucb$ helps to
% disambiguate between the effects of receding horizon control (vs. global
% heuristic planning) and those of global uncertainty reduction (vs. successive
% elimination).
We implement $\infomax$, a version of informative path planning in
\cite{marchant2014bayesian} specifically adapted for radioactive
source-seeking. %and summarized in Alg. \ref{alg:info_max}.
During each iteration of the algorithm, we solve an information maximization
problem over the space of trajectories ${\xi : [t, t + T_{\text{plan}}] \To
  \mc{B}}$ mapping from time in the next $T_{\text{plan}}$ seconds to a box
$\mc{B} \subset \mbb{R}^3$.
% These trajectories are encoded by second-order Bezier curves, which are
% paramaterized by the current position $p(t)$ of the sensor at time $t$ (which
% is known) and by two control points $p_1, p_2 \in \mc{B}$ for a total of six
% parameters.\footnote{Since the radiation sensor is directionally invariant,
% there is no need to optimize for orientation.} For clarity, we will denote
% these parameters as subscripts, e.g. $\tau_{p(t), p_1, p_2}(\cdot)$. Bezier
% curves provide a relatively low-dimensional representation of smooth
% trajectories, which are easier for a quadrotor to track, and they also provide
% a natural mechanism for encoding a velocity profile along the trajectory.

We measure the information content of a candidate trajectory $\xi$ by
accumulating the sensitivity-weighted variance at each grid point $x \in \calS$
at $N$ evenly-spaced times along $\xi$, i.e.
\begin{equation}
  \label{eqn:info_max}
  \xi^*_t = \arg \max_{\xi}  \sum_{i = 1}^N  \sum_{j = 1}^{|\calS|} \Sigma_{jj} \cdot h\left(x_j,\xi(t + T_{\text{plan}} i / N)\right) \enspace .
\end{equation}
This objective favors taking measurements sensitive to regions with high
uncertainty. As a consequence of the Poisson emissions model, these regions will
also generally have high expected intensity $\mu$; therefore we expect this
algorithm to perform well for $\RSS$. We parameterize
trajectories $\xi$ as second-order Bezier curves in $\RR^3$, and use Bayesian
optimization \cite{martinez2014bayesopt} to solve \eqref{eqn:info_max} because
of the high computational cost of evaluating the objective function.
% In particular, populating the values of the measurement matrix $\mbf{h}$ at
% each time $\{ t + \frac{i}{N} T_{\text{plan}} \}_{i=1}^N$ requires evaluating
% the sensor's sensitivity to every pixel in the grid.

% \subsubsection{$\naivesnake$}
% \label{subsubsec:uniform_sampling}


% simple scheme for solving our problem is to sample the space uniformly until
% some stopping criterion is satisfied. Since we represent the space as a grid,
% one natural approach to achieving such a uniform sample is to fly in a raster
% (`snake') pattern over the grid at the minimum allowable height.

% \subsection{Stopping Criteria and Metrics}

\textbf{Stopping criteria and metrics.} All three algorithms
use the same stopping criterion, which is satisfied when the highest LCB exceeds
the second-highest UCB. For sufficiently small $\delta$ the stopping criterion
ensures that the source is almost always correctly identified by all algorithms.
The source is always correctly identified in all experiments in Sec.
\ref{sec:results}.

% This gives a global measure of the accuracy of the predicted source emission
% rates in the grid.


% We expect the information gain approach to be superior with respect to this
% metric since it is based on a global information criterion rather, whereas our
% bandit-based algorithm takes measurements only in order to distinguish between
% the two most promising regions.
% \item Euclidean distance of estimated extremal point to true source point, in
%   Euclidean distance. This is a measure of how well we localize the source. We
%   expect both methods to perform well with respect to this metric since they
%   should both find the source eventually.

%   We expect our algorithm to outperform the baseline with respect to this
%   metric since the bandit logic should choose to sample the source pixel most
%   frequently, whereas the baseline information maximization approach will
%   cover the space more evenly.

%   We expect the bandit algorithm to run significantly more quickly than the
%   baseline.

%   \comment{We don't have $\alpha$ anymore...}


==> problem_formulation.tex <==




==> theorem_and_baby_proof_old.tex <==
%!TEX root = main_ieee.tex
\section{Theoretical Runtime and Sampling Analysis}
\label{sec:analysis}
We now present a theoretical analysis for $\snakeucb$ and $\naivesnake$ under the
pointwise sensing model from Sec.~\ref{sec:ptwise_ci}.
%, as they are more amenable
%to such analysis than $\infomax$. 
For simplicity, we
first present results for  $k = 1$ in Theorem~\ref{prop:sample_comp_simpler},
then state the corresponding results for $k \geq 1$ in Corollary~\ref{thm:snakeucb_runtime_topk_inmain}.
 \iftoggle{ieee}{}{Proofs, along with general results for arbitrary $k$, and complimentary lower bounds, are presented in Appendix~\ref{sec:main_theory_results}.}
 %Theorem~\ref{thm:snakeucb} in Appendix~\ref{sec:app_kone} gives a formal runtime bounds for $\snakeucb$ when $k = 1$, and Theorem~\ref{thm:snakeucb_runtime_topk} in Appendix~\ref{sec:app_genk} provides the general bound for $k \ge 1$.  Propositions~\ref{thm:naivesnake} and Theorem~\ref{thm:naivesnake_top_k}, in Appendices~\ref{sec:app_kone} and~\ref{sec:app_genk}, respectively, give formal runtime bounds for $\naivesnake$ for $k=1$ and $k \ge 1$, respectively. Finally, Proposition~\ref{prop:lower_bound} in Appendix~\ref{sec:app_kone} establishes lower bounds which show th{}at $\snakeucb$ (resp. $\naivesnake$) attain nearly optimal runtimes for adaptive (resp. passive) sampling.

Our analysis shows that both algorithms correctly identify the maximal source
with high probability and sharply quantifies the relative  advantage of
$\snakeucb$ over $\naivesnake$ in terms of the distribution of the background
radiation. The empirical results presented in Sec.~\ref{sec:results} validate the correctness of both algorithms and show that our theoretical results are indeed predictive of the relative performance of $\snakeucb$ and $\naivesnake$ in simulation.

%In the appendix, we complement the runtime analysis with a lower bound which shows that $\snakeucb$ nearly achieves the optimal runtime attainable by any adaptive sensing strategy, for the point-wise model.

We analyze $\snakeucb$ with the trajectory planning strategy outlined in
Sec.~\ref{sec:snake_path}. For $\naivesnake$, the robot spends time $\tau_i$ at
each point in each round $i$ until termination, which is determined by the same
confidence intervals and termination criterion for $\snakeucb$.

We will be concerned with the \emph{total runtime}, defined as
\begin{align*}
\Truntime &= \begin{cases}\sum_{i = 0}^{\ifin} \left(\tau_i|\calS_i| + \tau_0|\calS \setminus \calS_i|\right)  & (\snakeucb)\\
\sum_{i = 0}^{\ifin} \tau_i|\calS| & (\naivesnake)
\end{cases},
\end{align*}
where $\ifin$ denotes the round at which the algorithm terminates.  Since $k =
1$, we shall replace $\Sstk$ with $x^*$, with $\mu^* = \mu(x^*)$. Our bounds will be stated in terms of the divergences
% \iftoggle{ieee}
% {$\divergx := \frac{(\mu^* -  \mu(x))^2}{\mu^*}$
% }
{
\begin{align*}
\divergx := \frac{(\mu^* -  \mu(x))^2}{\mu^*},
\end{align*}
}which approximate the $\KL$-divergence between the distribution $\Poi(\mu^*)$
and $\Poi(\mu(x))$\iftoggle{ieee}{}{(see Appendix~\ref{sec:main_theory_results})}, and therefore the sample complexity of distinguishing between
the maximal source and
a source emitting photons at rate $\mu(x)$.
In general, one can define analogous divergences for any exponential family distribution.

\begin{theorem}(Sample and Runtime Guarantees for $k = 1$).
\label{prop:sample_comp_simpler}{}  Define the adaptive and uniform sample complexity terms $\Hadapt$ and $\Hunif$:
\iftoggle{ieee}
{
	\begin{align}
 \Hadapt &:= |\calS| \tau_0 + \sum_{x \in  \calS \setminus \{x^*\}}\left(
    \tfrac{1}{\divergx}\right) \nonumber \\
    \Hunif  &:= |\calS| \tau_0 + |\calS| \max_{x \in \calS}
  \tfrac{1}{\divergx}\label{eqn:complexity}~.
	\end{align}
}
{
	\begin{eqnarray}
 \Hadapt := \sum_{x \in  \calS \setminus \{x^*\}}\left( \tau_0 +
    \frac{1}{\divergx}\right) & \text{ and } &
    \Hunif  := |\calS| \left( \tau_0 + \max_{x \in \calS}
  \frac{1}{\divergx} \right)  \label{eqn:complexity}~.
\end{eqnarray}
}

Regardless of the distribution of the emitters, $ \Hadapt \leq \Hunif$. For any $\deltot \in (0,1)$, the following hold each with probability $1-\deltot$:
(i) $\snakeucb$ executed with confidence parameter $\deltot$ returns the correct maximal
source $x^*$ and satisfies the guarantee:
\iftoggle{ieee}
{
  \begin{align*}
\Truntime(\snakeucb) \le~&\Hadapt \cdot\BigOhTil\left(\log(|\calS|/\deltot\right)\\
                           &\quad+\BigOhTil\left(|\calS| \log(\Hunif / |\calS|)\right).  %\tag*{(\snakeucb)}.
\end{align*}
}
{
\begin{align*}
\Truntime(\snakeucb) \le \Hadapt \cdot
                           &\BigOhTil\left(\log(|\calS|/\deltot)\right) + \mathcal{O}(|\calS| \log(\Hunif / |\calS|).  %\tag*{(\snakeucb)}.
\end{align*}
}
 (ii) $\naivesnake$ executed with confidence parameter $\deltot$
returns the correct maximal source $x^*$ and satisfies the following guarantee:
% runtime $\Truntime$ of $\naviesnake$ is bounded as
\begin{align*}
\Truntime(\naivesnake) \le \Hunif \cdot
  \BigOhTil\left(\log(|\calS|/\deltot)\right).  %\tag*{(\naivesnake)}.
\end{align*}

\begin{proof}
(Sketch\iftoggle{ieee}{}
%see also Appendix~\zref{sec:main_theory_results} of \cite{rolf2018successive}
{; see also Appendix~\zref{sec:main_theory_results} of \cite{rolf2018successive}}).
\iftoggle{ieee}{
Consider a complete run of $\snakeucb$. For each point $x \in \calS$, let $\ifin(x)$ denote the round at which $\snakeucb$ removes $x$ from $\calS_i$; at this point we are confident as to whether or not $x$ is $x^*$, so we do not sample it on successive rounds. At round $i$, we spend time $\tau_i = 2^i$ sampling each point still in $\calS_i$, so that in total, we spend $\sum_{x \in \calS} \sum_{i=0}^{\ifin(x)}\tau_i \leq \sum_{x \in \calS} 2^{1 + \ifin(x)}$ time sampling. For $\naivesnake$, we sample all points in all rounds, so we spend time $\leq |\calS| \max_{x \in \calS} 2^{1 + \ifin(x)}$ sampling.
The additional traversal time for the entire run of each algorithm is the time it takes to traverse the grid, $|\calS| \tau_0$, multiplied by the total number of rounds  $ \max_{x \in \calS} \ifin(x) $.

It remains to bound $\ifin(x), x \in \calS$ for each algorithm, and establish correctness.  These quantities depend on the estimated means $\hat{\mu}_i(x)$. Using the same concentration bounds that informed the bounding functions in Sec.~\ref{sec:ptwise_ci}, we can deterministic bounds ${[\LCBbar_i, \UCBbar_i]}$ that depend only on the true means $\mu(x)$. We choose these bounds to encompass the algorithm confidence intervals, so that: $\LCBbar_i(x) \leq \LCB_i(x) \leq \mu(x) \leq \UCB_i(x) \leq \UCBbar_i(x)$ with high probability. If each separate inequality holds during a single round with probability $\deltot/(4|\calS|i^2)$, then a union bound gives that the probability of failure is at most $\deltot$. This ensures probabilistic correctness with probability at least $ 1-\deltot$ by application of Lemma~\ref{lem:main_correctness}.

Because $\LCBbar_i(x)$ and $\UCBbar_i(x)$ are deterministic given $\mu(x)$ and are contracting to $\mu(x)$ nearly geometrically in $i$, we can bound $\ifin(x)$ by inverting the intervals to find the smallest integer $i$ such that
$\LCBbar_i(x^*)$ is larger than $\UCBbar_i(x)$ for any other $x \in \calS \setminus x^*$.
This requires an inversion lemma from the best arm identification literature (Equation (110) in \cite{simchowitz2016best}). The specific forms of $\LCBbar_i$ and $\UCBbar_i$, yield the bounds on $\ifin(x)$ in terms of approximate KL divergences in~\eqref{eqn:complexity}.
}
{See Appendix~\ref{sec:main_theory_results}}
\end{proof}
\end{theorem}

In order to extend the results of Theorem~\ref{prop:sample_comp_simpler} to the more general $k\geq 1$ setting,
we must consider the divergence terms not between emitters x and the maximum emitter $x^*$, but rather the divergences with respect to the $k^{\mathrm{th}}$ and $(k+1)^{\mathrm{th}}$ emitters:
\begin{align*}
  \divergtop &= \frac{(\mu(x) - \mu^{(k+1)})^2}{\mu(x)},~(\mu(x) > \mu^{(k+1)})  \quad \text{and } \quad\\%\\\text{ for}~ \mu(x) > \mu^{(k+1)} \quad \text{and}\\
  \divergbot &= \frac{(\mu^{(k)} - \mu(x))^2}{\mu^{(k)}},\quad (\mu(x) < \mu^{(k)}).%,\text{ for}~ \mu(x) < \mu^{(k)}
\end{align*}

For $x \in \calS^*(k)$, $\divergtop$ describes how close the emission rate $\mu(x)$ is to the ``best'' alternative in $\calS \setminus \calS^*(k)$. For $x \in \calS \setminus \calS^*(k)$, $\divergbot$ describes how close $\mu(x)$ is to the mean $\mu^{(k)}$ of the emitter in $\calS^*(k)$ from which it is hardest to distinguish.

\begin{corollary}(Sample and Runtime Guarantees for $k \geq 1$).
  \label{thm:snakeucb_runtime_topk_inmain}
  Define the general adaptive and uniform sample complexity terms $\Hadaptk$ and $\Hunifk$ for any integer $k \geq 1$:
\begin{eqnarray}
\label{eq:sample_complexity_k}
\Hadaptk &:=& |S|\tau_0 + \sum_{x \in \calS^*(k)} \tfrac{1}{\divergtop} + \sum_{x
              \in \calS \setminus \calS^*(k)} \tfrac{1}{\divergbot} \nonumber\\
\Hunifk &:=& |\calS| \tau_0 + |\calS| \frac{1}{\diverg(\mu^{(k+1)}),\mu^{(k)})}
\end{eqnarray}

$\Hadaptk \geq \Hunifk$ for any number of sources $k$ and distribution of emitters. For any $\deltot \in (0,1)$, the following hold each with probability at least $1-\delta$:  \\
(i)
$\snakeucb$ correctly returns $\Sstk$,
  and the total runtime is bounded by
   \begin{align*}
    \Truntime(\snakeucb) \leq~& \Hadaptk \cdot
    %\Tsample + \cardS \log_+ \left(\frac{\log_+\tfrac{\cardS}{\delta}}{\diverg(\mu^{(k+1)},\mu^{(k)})} \right) ~=~
    \BigOhTil\left( \log ({\cardS}/ {\deltot})\right) \\
    &\quad+\BigOhTil\left(\cardS \log_+\left( {\Hunifk}/ {\cardS}\right)\right)~.
    %&=& \calO\left(\Hadapt\log(M/\delta) + \tau_0 M^2 \log(\Hunif)\right)~.
  \end{align*}
  (ii) $\naivesnake$ correctly returns $\Sstk$, and the total runtime is bounded above by
  \begin{eqnarray*}
   \Truntime(\naivesnake) \leq  \Hunifk \cdot \BigOhTil\left(\log(\cardS/\deltot)\right)~.
  \end{eqnarray*}
\begin{proof}(Sketch).
We obtain the same deterministic confidence intervals for each point $x \in S$ at each iteration $i$,  $\LCBbar_i(x)$ and $\UCBbar_i(x)$, as in the proof of~Theorem~\ref{prop:sample_comp_simpler}.
However, for $k>1$, we need to separate slightly different confidence intervals. That is, for every $x$ with $\mu(x) < \mu^{(k+1)}(x)$, we must ensure $\UCBbar_i(x) < \LCBbar_i(x^{(k)})$ at $i=\ifin$ (and thus nothing will be returned in $\calS^*(k)$ that doesn't belong). Similarly, for every $x$ with $\mu(x) < \mu^{(k+1)}(x)$, we need $\LCBbar_i(x) > \UCBbar_i(x^{(k+1)})$, ensuring everything that belongs in $\calS^*(k)$ is included.

Using the same bounding techniques as in~Theorem~\ref{prop:sample_comp_simpler} yields the sample complexity bounds in~\eqref{eq:sample_complexity_k}. The form of $\Hunifk$ results from noting that the function $(a,b) \mapsto \frac{a}{(a - b)^2}$ is decreasing in $a$ and increasing in $b$ for $a > b$, and therefore
$
\max\left\{\max_{x \in \calS^*(k)} \frac{1}{\divergtop},    \max_{x \in \calS \setminus \calS^*(k)} \frac{1}{\divergbot}\right\} =  \diverg(\mu^{(k+1)}),\mu^{(k)}).
$
  \end{proof}
\end{corollary}

The $\BigOhTil\left(\log(|\calS|/\deltot)\right)$ term in the $\snakeucb$ runtime bounds accounts for travel times of transitioning between measurement configurations. The second term $|\calS| \log(\Hunif / |\calS|)$
%in the expression for $\Truntime(\snakeucb)$
accounts for the travel time of traversing the uninformative points in the global path $\trajpoints$ at a high speed.
Observe that this term is never larger than the term $\Truntime(\naivesnake)$ and is typically dominated by ${\Hadapt\cdot \BigOhTil\left(\log(|\calS|/\deltot)\right)}$.
With a uniform strategy, the number of measurements (and hence the total
time) scales with the \emph{largest value} of $1/\divergx$ over $x \in
\calS$ because that quantity alone determines the number of rounds required. In
contrast, $\snakeucb$ scales with the \emph{average} of $1/\divergx$ because it dynamically chooses
which regions to sample more precisely. In an experimental setting, we validate that when the
values of $\divergx$ are heterogeneous, $\snakeucb$ yields
significant speedups over $\naivesnake$ (Fig.~\ref{fig:comparison_results}). \esther{TODO: mention here the expected runtimes that we use in figure 3}


We remark that our sample complexity results qualitatively match standard bounds for
  active top-$k$ identification with sub-Gaussian rewards in the general
  multi-armed bandit setting (e.g., ~\cite{kalyanakrishnan2012pac}).


==> top_k_proofs.tex <==
%!TEX root = appendix_nips.tex
\section{Proof of Theorem~\ref{thm:snakeucb_runtime_topk} For Top-$k$ \label{sec:topkproof}}
In this section, we sketch the Proof of Theorem~\ref{thm:snakeucb_runtime_topk}. The proof is very similar to those of Theorem~\ref{thm:snakeucb} and Proposition~\ref{thm:snakeucb_runtime}, so we will focus on highlighting the major differences and added nuances. As in Proposition~\ref{thm:snakeucb_runtime}, the total run time is bounded by
\begin{eqnarray}
\tau_0\cardS \sum_{i \ge 0} \I(|\calS_i| + |\Stop_i| > k) +  \sum_{i \ge 0} 2^{i} |\calS_i| \I(|\calS_i| + |\Stop_i| > k)
\end{eqnarray}
Hence, our goal is to bound both the total number of rounds $\sum_{i \ge 0} \I(|\calS_i| + |\Stop_i| > k$, as well as the sample complexity $\sum_{i \ge 0} 2^{i} |\calS_i| \I(|\calS_i| + |\Stop_i| > k) $. We begin by observing that Lemma~\ref{lem:egood}, which states the event $\Egood$ defined as
\begin{eqnarray}
\forall i \ge 1, x \in \calS_i : \LCBbar_i(x) \le \LCB_i(x) \le \mu(x) \le \UCB_i(x) \le \UCBbar_i(x)~,
\end{eqnarray}
still holds with probability $1-\delta$ for the top-$k$ version of $\snakeucb$. 

	The following lemma is at the heart of our analysis:
	\begin{lemma}\label{lemtop_k_correct} $\Stop_i$ and $\calSi$ are disjoint for all rounds $i$. Moreover, suppose that for all rounds $i$ and all $x \in \calS_i$, the confidence intervals satisfy $\LCB_i(x) \le \mu(x) \le \UCB_i(x)$. Then $\Stop_i \subset \calS^*(k)$, and $\calS^*(k) \setminus \Stop_i \subset \calS_i$.
	\end{lemma}
	In other words, the update rules only add to $\Stop_i$ elements which are certain to be among the top-$k$, and only remove from $\calS_i$ elements which are certain to be ruled out from the top-$k$. Lemma~\ref{lemtop_k_correct} is proved in Sec.~\ref{proof_lemtop_k_correct}. In particular, on $\Egood$, we always have $\calS^*(k) \subset \calS_i \cup \Stop_i$, so that when the termination criterion $|\Stop_i| + |\calS_i| \le k$ occurs, $\Stop_i \cup \calS_i = \calS^*(k)$. This gives correctness under the event $\Egood$.

To analyze the stopping time, we first note that the quantities $\LCBbar_i(x)$ and $\UCBbar_i(x)$ are deterministic, and depend only on $\mu(x)$. Hence, we can define $\LCBbar_i^{(k)}$ and $\UCBbar_i^{(k+1)}$ to denote $\LCBbar_i(x^{+})$ and $\UCBbar_i(x^{(i)})$ for any $x^+,x^-$ with $\mu(x^+) \ge \mu^{(k)}$ and $\mu(x^-) \le \mu^{(k+1)}$.
\begin{lemma}\label{lemma:run_time_egood} Suppose that $\Egood$ holds, and $x \in \calS_i$. Then either $|\calS_i| + |\Stop_i| = k$ or $|\calS_i| + |\Stop_{i+1}| = k$, or otherwise $x \notin \calS_{i+1}$ as long as
\begin{eqnarray}
\begin{cases}
\LCBbar_i(x) > \UCBbar_i^{(k+1)} & \mu(x) \ge \mu(x^{(k)}) \\
\UCBbar_i(x) < \LCBbar_i^{(k)} & \mu(x) \le \mu(x^{(k+1)}) \\
\end{cases}
\end{eqnarray}
\end{lemma}
Since $\LCBbar$ and $\UCBbar$ are deterministic quantities, Lemma~\ref{lemma:run_time_egood} implies a deterministic upper bound on run-time under $\Egood$. Indeed, the total sample complexity is bounded by
\begin{eqnarray*}
&&\sum_{i \ge 0} 2^{i} |\calS_i| \I(|\calS_i| + |\Stop_i| > k) \le  \\
&&2\sum_{x \in \calS^*(k)} \inf\{2^i : \LCBbar_{i}(x) > \UCBbar^{(k+1)}_{i}(x)\}~ + 2\sum_{x \in \calS \setminus \calS^*(k)} \inf\{2^i : \UCBbar_{i}(x) < \LCBbar^{(k)}_{i}(x)\}~
\end{eqnarray*}
For $x \in \calS^*(k)$, we apply Proposition~\ref{prop:sample_comp} with $x_1 = x$ and $x_2$ such that $\mu(x_2) = \mu(x^{(k+1)})$. This gives that for any $x \in \calS^*(k)$,
\begin{eqnarray}\label{}
\inf\{2^i : \LCBbar_{i}(x) > \UCBbar^{(k+1)}_{i}(x)\} \lesssim C \left(\tau_0 + \frac{\mu(x) \log_+\left(\cardS \log_+\left(\frac{\mu(x)}{\Delta_{x;k}}\right)/\delta\right)}{\Delta_{x;k}^2}\right)
 \end{eqnarray}
and for any $x \in \calS \setminus \calS^*(k)$,
\begin{eqnarray}
 \inf\{2^i : \UCBbar_{i}(x) < \LCBbar^{(k)}_{i}(x)\} \lesssim C \left(\tau_0 + \frac{\mu^{(k)} \log_+\left(\cardS \log_+\left(\frac{\mu^{(k)}}{\Delta_{x;k}^2}\right)/\delta\right)}{\Delta_{x;k}^2}\right)
\end{eqnarray}
Summing the above two equations yields the first two terms in the bound given in Theorem~\ref{thm:snakeucb_runtime_topk}. For the last equation, we observe that by Lemma~\ref{lemma:run_time_egood}, the total number of rounds is given by
\begin{eqnarray*}
&&\max \left\{ \max_{x \in \calS \setminus \calS^*(k)}\inf \{i: \UCBbar_i(x) < \LCBbar_i^{(k)}\} , \max_{x \in \calS^*(k)}\inf \{i: \LCBbar_i(x) > \UCBbar_i^{(k+1)}\}  \right\} \\
&=& \max \left\{ \inf \{i: \UCBbar_i^{(k+1)} < \LCBbar_i^{(k)}\}, \inf \{i: \LCBbar_i^{(k)} > \UCBbar_i^{(k+1)}\}  \right\} \\
&=& \inf \{i: \UCBbar_i^{(k+1)} < \LCBbar_i^{(k)}\}\\
&\le&C \log \left(\tau_0 + \frac{\mu^{(k)} \log_+\left(\cardS \log_+\left(\frac{\mu^{(k)}}{(\mu^{(k)} - \mu^{(k+1)})^2}\right)/\delta\right)}{(\mu^{(k)} - \mu^{(k+1)})^2}\right)\\
&=& C \max_{x \notin \calS^*(k)}\log \left(\tau_0 + \frac{\mu^{(k)} \log_+\left(\cardS \log_+\left(\frac{\mu^{(k)}}{\Delta_{x;k}^2}\right)/\delta\right)}{\Delta_{x;k}^2}\right)~.
\end{eqnarray*}
Putting the pieces together concludes the proof.



\subsection{Proof of Lemma~\ref{lemma:run_time_egood}}
Let us first consider $x \in \calS_i$ with $\mu(x) \ge \mu^{(k)}$. Suppose $\Egood$ holds and $|\calS_i| > k - |\Stop_i|$ Then, there exists a point $x_- \in \calS_i \cap \{\calS \setminus \calS^*(k)\}$. Then $\mu(x_-) \le \mu^{(k+1)}$.  Since $\UCBbar_{i+1}(x)$ are monotone functions of $\mu(x)$, one has
\begin{eqnarray}
\UCB_{i}(x_-) \le \UCBbar_i(x_-) \le  \UCBbar_i^{(k+1)}
\end{eqnarray}
In particular, we find that
\begin{eqnarray}
	\mathrm{max}_{x' \in \calS_i}^{(k+1 - |\Stop_i|)} \UCB_{i}(x') \le \UCBbar_{i}^{(k+1)}
\end{eqnarray}
Hence, as soon as $\LCBbar_i(x) > \UCBbar_{i}^{(k+1)}$, 
\begin{eqnarray}
 \LCB_i(x) \ge \LCBbar_i(x) >  \UCBbar_{i}^{(k+1)} \ge \mathrm{max}_{x' \in \calS_i}^{(k+1 - |\Stop_i|)} \UCB_{i}(x')~,
	\end{eqnarray}
	so $x$ is removed from $\calS_i$ and placed in $\Stop_i$ by Equations~(\zref{eq:top_elim}) and~(\zref{eq:bot_elim}) in the main text.

Now consider $x \in \calS_i$ and $\mu(x) \le \mu^{(k+1)}$, and suppose that $|\calS_i| > k - |\Stop_{i+1}|$. Then there is an $x_+ \in \calS_i \cap \calS^*(k)$; $\mu(x_+) \ge \mu(x^{(k)}$, and thus $\LCB_i(x_+) \ge \LCBbar_i(x_+) \ge \LCBbar^{(k)}_i$. Thus, as soon as $\UCBbar_i(x) < \LCBbar_{i}^{(k)}$, then
\begin{eqnarray}
 \UCB_i(x) \le \LCBbar_i(x) <  \LCBbar_{i}^{(k+1)} \le \mathrm{max}_{x' \in \calS_i - \Stop_{i+1}}^{(k - |\Stop_{i+1}|)} \LCB_{i}(x')\}  ~,
	\end{eqnarray}
	so $x$ is removed from $\calS_i$ by Equation~(\zref{eq:bot_elim}) in the main text.

\subsection{Proof of Lemma~\ref{lemtop_k_correct}} \label{proof_lemtop_k_correct}
	Assume inductively that with high probability over all rounds $i$ and all sources $x$, all elements of $\Stop_i$ are confidently among the top $k$ sources $\calS^*(k)$, and all elements of $\calS^*(k) \setminus \Stop_i$ are elements of the candidate set $\calS_i$. We will also use the notation $\max^{(j)} \{\cdot\}$ to denote the $j$-th largest element of the set $\{\cdot\}$.

	We may assume that $|\calS_i \cup \Stop_i| > k$.

	Let's first examine the update rule for $\Stop_i$. Under the assumption that $\LCB_i(x) \le \mu(x) \le \UCB_i(x)$ holds for all $x \in \calS_i$, we have that if $x \in \Stop_{i+1} \setminus \Stop_i$,
	\begin{eqnarray}
	\mu(x) \ge \LCB_i(x) > \mathrm{max}_{x' \in \calS_i}^{(k+1 - |\Stop_i|)} \UCB_{i+1}(x') \ge \mathrm{max}_{x' \in \calS_i}^{(k+1 - |\Stop_i|)} \mu(x')~.
	\end{eqnarray}
	This implies that $\mu(x)$ is greater than at least $\mu(x')$ for at least $|\calS_i| - (k - |\Stop_i|)$ elements $x' \in \calS_i$. Since there are precisely $|\calS_i| - (k - |\Stop_i|)$ members of $\calS_i$ which are in $\calS \setminus \calS^*(k)$, and these have the lowest means, the above conditions imply that $x$ is indeed in $\calS^*(k)$.

	Now let's examine the update rule for $\calS_i$. For ease of notation, define $\calS_i' := \calS_i \setminus \Stop_{i+1}$. If the confidence intervals are uniformly correct, then we have that if $x \in \Stop_{i+1} \setminus \calS'_i$,
	\begin{eqnarray}
	\mu(x) \le \UCB_i(x) < \mathrm{max}_{x' \in \calS_i'}^{(k - |\Stop_{i+1}|)} \LCB_{i+1}(x') \le \mathrm{max}_{x' \in \calS_i'}^{(k - |\Stop_{i+1}|)} \mu(x')~.
	\end{eqnarray}
	Thus, $\mu(x)$ is not among the top $k - |\Stop_{i+1}|$ true means in $\calS'$; and the $k - |\Stop_{i+1}|$ members of $\calS_i'$ which have the top means are precisely the elements of $\calS_i \cap \calS^*(k)$.

